Temporal Logics for Hyperproperties

Two new logics for verification of hyperproperties are proposed. Hyperproperties characterize security policies, such as noninterference, as a property of sets of computation paths. Standard temporal logics such as LTL, CTL, and CTL* can refer only to a single path at a time, hence cannot express many hyperproperties of interest. The logics proposed here, HyperLTL and HyperCTL*, add explicit and simultaneous quantification over multiple paths to LTL and to CTL*. This kind of quantification enables expression of hyperproperties. A model checking algorithm for the proposed logics is given. For a fragment of HyperLTL, a prototype model checker has been implemented.

==> SecLTL.tex <==
\section{HyperCTL}
\label{sect:logic}

In this section, we introduce HyperCTL, our extension of the temporal
logic CTL* for hyperproperties. We begin with a quick review of
standard notation for Kripke structures.

\subsection{Preliminaries: Kripke structures}
\label{sect:preliminaries}

A \emph{Kripke structure} $K=(S,s_0,\delta,\AP,L)$ consists of a set
of \emph{states} $S$, an \emph{initial state} $s_0\in S$, a transition
function $\delta:S\to 2^{S}$, a set of \emph{atomic propositions}
$\AP$, and a labeling function $L:S\to 2^{\AP}$.  We require that all
states $s\in S$ have at least one successor,
$\delta(s)\not=\emptyset$.  The \emph{cardinality} or \emph{size} of a
Kripke structure is defined as the cardinality of its states and
transitions $|K|= |S|\cdot|\AP|+|\delta|$, where $\delta$ is
interpreted as a set of tuples.
%
A \emph{path} $\pi\in (S\times2^\AP)^{\omega}$ is an infinite sequence
of labeled states (i.e., states equipped with a set of atomic
propositions).
%
For a path $\pi$ and $i \in \mathbb N$, $\pi(i)$ is the $i$-th state
of the sequence and $\pi[i]$ is the $i$-th set of atomic propositions.
Furthermore, we use $\pi[0,i]$ to denote the prefix of $\pi$ up to
(including) position $i$, and $\pi[i,\infty]$ to denote the suffix starting
at position $i$.  We lift these notions to tuples of paths by applying
the operations for each position:
e.g. $\langle\pi_1,\dots,\pi_n\rangle[i,\infty]=\langle\pi_1[i,\infty],\dots,\pi_n[i,\infty]\rangle$.
Every Kripke structure $K$ gives rise to a set of paths from any state
$s\in S$, denoted by
$\Paths_{K,s}$. %; for the initial state $s_0$, we define $\Paths_{K}=\Paths_{K,s_0}$.
%As usual, a Kripke structure $K$ generates a set of paths, which we will denote with $\Paths_K$, and we will use an index $s$, e.g. $\Paths_{K,s}$, to denote all its postfixes of paths in $\Paths_K$ that start with the state~$s$. 
%
To allow the case of a specification referring to atomic
propositions that are not contained in the atomic propositions $\AP$
of the Kripke structure, we assume that these atomic propositions are
not restricted.
%
Therefore, we define 
%
\(
\Paths_{K,s}^{\AP'}=\big\{(s_1,P_1\cup P'_1).(s_2,P_2 \cup P'_2).\dots ~\mid~ (s_1,P_1).(s_2,P_2).\dots\in\Paths_{K,s},~ \forall i.~P'_i\subseteq \AP'\setminus\AP\big\}. \)



\subsection{Syntax}

%\paragraph*{HyperCTL} 
We extend the syntax of CTL* with path variables. Path variables are introduced by path quantifiers. Since formulas may refer to multiple paths at the same time, 
atomic propositions are indexed with the path variable they refer to.
%
%With this work, we revisit quantification over paths in temporal logics. 
%The semantics of linear time logics, such as LTL, rely on a single quantification over the paths of the system and also branching time logics severely limit the use of quantifiers. 
%For example, CTL* restricts the scope of its variables such that the labels can only refer to the least recently introduced path. 
%We lift this restriction and allow to introduce multiple paths with different names and to refer to their labels later on. 
%This enables us to refer to multiple paths at once and, especially, to compare them to another. 
%For example, we can specify that there is at most one trace in a system, that is that there are no two different paths: $\neg\exists\pi_1,\pi_2.~\pi_1\not=\pi_2$\;. 
%
%Let $\AP$ be a set of atomic propositions and let $\mathcal V$ be an infinite supply of path variables.
The formulas of HyperCTL are defined by the following grammar, where
$a\in\AP$ for some set $\AP$ of atomic propositions and $\pi \in
\V$ for an infinite supply $\V$ of path variables:
%
%This leads to the logics HyperLTL and HyperCTL that are defined by the grammar 
\[
\quad\quad\quad\varphi ~ ::= \quad~ a_{\pi} \quad~ \vert \quad~ \neg\varphi \quad~ \vert \quad~ 
\varphi\vee\varphi
\quad~ \vert \quad~ \LTLcircle\varphi \quad~ \vert \quad~ \varphi \U\varphi %\quad~ \vert \quad~ \varphi \R \varphi 
%\quad~\vert\quad~ \S \varphi
\quad~ \vert \quad~ \exists \pi.\; \varphi 
\]
%
A formula is \emph{closed} if all occurrences of some path variable
$\pi$ are in the scope of a path quantifier $\exists \pi$. A HyperCTL
\emph{specification} is a Boolean combination of closed HyperCTL
formulas each beginning with a quantifier (or its negation). A formula
is in \emph{negation normal form} (NNF) if it only contains negations
in front of labels and in front of quantifiers. Every HyperCTL formula
can be transformed into an equivalent formula in negation normal form,
if we introduce the additional operators
$\varphi_1\wedge\varphi_2\equiv \neg(\neg\varphi_1\vee\neg\varphi_2)$
and $\varphi_1\R\varphi_2\equiv \neg(\neg\varphi_1\U\neg\varphi_2)$.

We extend HyperCTL with \emph{universal} path quantification
$\forall\pi.\;\varphi \equiv \neg\exists\pi.\neg\varphi$ as well as
with the usual temporal operators: $\true\equiv a_\pi\vee\neg a_\pi$,
$\false\equiv\neg\true$, $\LTLdiamond\varphi\equiv\true\U\varphi$,
$\LTLsquare\varphi\equiv\neg\LTLdiamond\neg\varphi$,
$\varphi_1\W\varphi_2\equiv\varphi_1\U\varphi_2\vee\LTLsquare\varphi_1$.
For convenience, we also introduce some abbreviations for comparing
paths.  Given a set $P\subseteq \AP$ of atomic propositions, we
abbreviate $\pi[0]\!=_P\!\pi'[0] ~\equiv~ \bigwedge_{a\in P}
a_{\pi}\!\leftrightarrow\! a_{\pi'}$, and $\;\pi\!=_P\!\pi' ~\equiv~
\LTLsquare (\pi[0]\!=_P\!\pi'[0])$, and analogously for $\neq$, e.g.,
$\pi\!\neq_P\!\pi'~\equiv~\neg(\pi\!=_P\!\pi')$.
%If $P = \AP$, we omit $P$:
%%Comparison without a set $P$ denotes the identity on $\AP$:  
%$\pi[0]\!=\!\pi'[0]~\equiv~\pi[0]\!=_{\AP}\!\pi'[0]$.
%
Finally, %we introduce $\alpha$-conversion for atomic propositions as a syntactic operation on formulas:
$[\varphi]_\pi$ indicates that the atomic propositions in $\varphi$
are indexed with the path variable $\pi$, and $[\varphi]_{\pi\to
  \pi'}$ is the formula obtained by replacing index $\pi$ by index
$\pi'$ on all (free) atomic propositions in $\varphi$.
%all atomic propositions in $\varphi$ that are indexed with path variable $\pi$ are now indexed with path variable $\pi'$. 


%We assume that temporal operators are only used after at least one path has been introduced and that 

%\paragraph*{HyperLTL} HyperLTL is the restriction of HyperCTL where no path quantifiers occur after a temporal operator.
%Quantifiers in HyperLTL thus only refer to the paths starting in the initial state and do not further restrict the branching of the Kripke structure.

%do not restrict the branching of the system, but only refers to paths starting from the initial states of the system. 
%Thus, it captures the fragment of ``non-branching time'' hyperproperties expressible by HyperCTL and includes most of the examples we give in this work. 
%An example that inherently requires both, the branching time view and the comparison of paths,  will be discussed in Subsection~\ref{ssect:declassification}. 
%



\subsection{Semantics}
 
Let $K = (S,s_0,\delta,\AP,L)$ be a Kripke structure and $\varphi$ a
HyperCTL formula over atomic propositions $\AP'$.
%
We define $\Pi\models_K\varphi$, the satisfaction relation of $\varphi$
with respect to a set of paths $\Pi=\tupleof{\pi_1,\dots,\pi_m}$, as follows:
\[
\begin{array}{l@{\hspace{1.5em}}c@{\hspace{1.5em}}l}
  \Pi\models_K a_{\pi_k} & \text{whenever} & a\in \pi_k[0] \\
  \Pi\models_K \neg \psi & \text{whenever} & \Pi\not\models_K\psi \\
  \Pi\models_K \psi_1 \vee \psi_2 & \text{whenever} & \Pi\models_K\psi_1 \text{ or } \Pi\models\psi_2 \\
  \Pi\models_K\LTLcircle\psi & \text{whenever} & \Pi[1,\infty]\models_K\psi  \\
  \Pi\models_K\psi_1\Until\psi_2 & \text{whenever} & \exists i \geq 0.~ \Pi[i,\infty]\models_K\psi_2 \;\;\;\text{and}\;\;\;
%\text{and}\\ &&
\forall 0 \leq j < i.~ \Pi[j,\infty]\models_K\psi_1  \\
%\text{if } \varphi = \psi_1\mc R\psi_2 & \text{then} & \forall i \geq 0.~ \Pi[i,\infty]\models_K\psi_2 \; \text{ or}\\
%&& \exists 0 \leq j < i.~ \Pi[j,\infty]\models_K\psi_1 \;, \\
   \Pi\models_K\exists\pi.\; \psi & \text{whenever} & \exists \pi\in\Paths_{K,\pi_n[0]}^{\AP'}.~ \Pi+\pi\models_K\psi \;,
\end{array}
\]
%
% \[
% \begin{array}{lcl}
%   \Pi\models a_{\pi_k} & \text{whenever} && a\in \pi_k[0] \;, \\
% \text{if } \varphi = \neg \psi & \text{then} & \Pi\not\models_K\psi \;,\\
% \text{if } \varphi = \psi_1 \vee \psi_2 \!\!\!& \text{then} & \Pi\models_K\psi_1 \text{ or } \Pi\models\psi_2 \;,\\
% \text{if } \varphi = \LTLcircle\psi & \text{then} & \Pi[1,\infty]\models_K\psi \;, \\
% \text{if } \varphi = \psi_1\mc U\psi_2 & \text{then} & \exists i \geq 0.~ \Pi[i,\infty]\models_K\psi_2 \; \text{ and}\\
% && \forall 0 \leq j < i.~ \Pi[j,\infty]\models_K\psi_1 \;, \\
% %\text{if } \varphi = \psi_1\mc R\psi_2 & \text{then} & \forall i \geq 0.~ \Pi[i,\infty]\models_K\psi_2 \; \text{ or}\\
% %&& \exists 0 \leq j < i.~ \Pi[j,\infty]\models_K\psi_1 \;, \\
% \text{if } \varphi = \exists\pi.\; \psi & \text{then} & \exists \pi\in\Paths_{K,\pi_n[0]}^{\AP'}.~ \Pi+\pi\models_K\psi \;,
% \end{array}
% \]
%
%
where $\Pi+\pi$ is short for $\langle\pi_1,\dots,\pi_n,\pi\rangle$. For the special case that the set of paths is empty, $\Pi=\langle\rangle$, we set
$\Paths_{K,\pi_n[0]}=\Paths_{K,s_0}$.  We say that a Kripke structure
$K$ \emph{satisfies} a HyperCTL formula $\varphi$, denoted as $K\models
\varphi$, if $\langle\rangle \models_K \varphi$ holds true.  The
\emph{model checking problem} for HyperCTL is to decide
whether a given Kripke structure satisfies a given HyperCTL formula.

%To be able to transform any HyperCTL formula in NNF, we introduce the \emph{release} operator, $\R$, the dual of until: $\neg(\varphi\U\varphi')\equiv\neg\varphi\R\neg\varphi'$. 

%\begin{example}
%The independence of one set of propositions $A$ from another $B$, which is called \emph{noninterference} in security literature, can be seen as a prototype of hyperproperties: 
%\[
	%\forall \pi.~ \forall\pi'.~ \pi\!=_{\AP\setminus B}\! \pi' ~\to~ \pi\!=_{A}\!\pi'~.
%\]
%For more applications of HyperCTL, we refer to Sections~\ref{sect:ExamplesSecurity} and~\ref{sect:ExamplesCodingTheory}. 
%\end{example}

%\subsection{HyperCTL and Abstractions}
%
%When building a model from an actual system, we have to consider which properties are compatible with the abstraction techniques we apply. 
%Trace inclusion is one of the most basic requirements on abstraction techniques, but it suffices to enable fundamental approaches such as counterexample guided abstraction refinement. 
%An important question is, thus, whether the properties of our specification language are compatible with the trace inclusion relation between models; that is, whether a property that holds on one model, also holds on all models that allow for less paths. 
%In security literature such properties are often called to be preserved under refinement. 
%
%\begin{proposition}
%All HyperCTL properties that, in NNF, have only negated quantifiers (that is, have only $\forall$ quantifiers) are preserved under refinement. 
%\end{proposition}




==> ctl.tex <==
% !TEX root = paper.tex

\section{The insufficiency of branching-time logic}
\label{sec:whynotctl}

CTL and CTL$^*$ have explicit path quantifiers.  
It's tempting to try to express security policies with those quantifiers.
Unfortunately, that doesn't work for information-flow policies such as observational determinism~\eqref{hp:od}.
Consider the following fragment of CTL$^*$ semantics~\cite{Emerson+Halpern/1986/BranchingVersusLinearTimeTemporalLogic}:
\begin{equation*}
\begin{array}{ll}
s \models \A \phi &~\text{iff for all $\pi \in M$, if $\pi(1) = s$ then $\pi \models \phi$} \\
\pi \models \Phi &~\text{iff $\pi(1) \models \Phi$}
%\pi \models p &~\text{iff $p \in L(s)$} \\
\end{array}
\end{equation*}
\emph{Path formulas} $\phi$ are modeled by paths $\pi$, and \emph{state} formulas $\Phi$ are modeled by states $s$.
Set $M$ is all paths in the model.
State formula $\A \phi$ holds at state $s$ when all paths proceeding from $s$ satisfy $\phi$.
Any state formula $\Phi$ can be treated as a path formula, in which case $\Phi$ holds of the path iff $\Phi$ hold of the first state on that path.
Using this semantics, consider the meaning of $\AAx \phi$, which is the form of observational determinism~\eqref{hp:od}:
\begin{equation*}
\begin{array}{l}
s \models \AAx \phi \\
= \text{for all $\pi \in M$ if $\pi(1)=s$ then $\pi \models \A \phi$} \\
= \text{for all $\pi \in M$ and $\pi' \in M$, if $\pi(1)=\pi'(1)=s$ then $\pi' \models \phi$} 
\end{array}
\end{equation*}
Note how the meaning of $\AAx \phi$ is ultimately determined by the meaning of $\phi$, where $\phi$ is modeled by the single trace $\pi'$.  
Trace $\pi$ is ignored in determining the meaning of $\phi$;
the second universal path quantifier causes $\pi$ to ``leave scope.''
Hence $\phi$ cannot express correlations between $\pi$ and $\pi'$, as observational determinism requires.
So CTL$^*$ path quantifiers do not suffice to express information-flow policies.
Neither do CTL path quantifiers, because CTL is a sub-logic of CTL$^*$.
Self-composition does enable expression of some, though not all, information-flow policies in branching-time logics, as we discuss in \S\ref{sec:relatedlogics}.

==> fig.purge.tex <==
\begin{figure}[t]
\setlength{\unitlength}{1mm}
	\centering
	\begin{picture}(50,25)%[width=6cm]
		\put(-12,9){$\purge(\pi)$}
	
		\put(10,10){\circle*{1}}
		\put(24,10){\circle*{1}}
		\put(38,10){\circle*{1}}
%		\put(40,10){\circle*{1}}
		\put(49,10){\dots}

		\put(11,10){\line(1,0){12}}
		\put(25,10){\line(1,0){12}}
		\put(39,10){\line(1,0){5}}

		\put(5,13){$(\lambda,l)$}
		\put(19,13){$(\lambda,l)$}
		\put(33,13){$(\lambda,l')$}
%		\put(39,13){$(\lambda,l_2)$}

		\put(-1,24){$\pi$}

		\put(10,25){\circle*{1}}
		\put(24,25){\circle*{1}}
		\put(38,25){\circle*{1}}
%		\put(40,25){\circle*{1}}
		\put(49,25){\dots}

		\put(11,25){\line(1,0){12}}
		\put(25,25){\line(1,0){12}}
		\put(39,25){\line(1,0){5}}

		\put(5,28){$(h',l)$}
		\put(19,28){$(h'',l)$}
		\put(33,28){$(h''',l')$}
%		\put(39,28){$(l_2,h_3)$}

	\end{picture}
	\caption{Paths $\pi$ and $\purge(\pi)$ have the same low inputs and outputs, but $\purge(\pi)$ has empty high inputs and outputs.\label{fig:noninterference}}
\end{figure}

==> hp.tex <==
% !TEX root = paper.tex

\section{Hyperproperties in HyperLTL}
\label{sec:hp}

We've seen that HyperLTL can express many interesting security policies.
But what is the exact class of hyperproperties that can be expressed in HyperLTL?
It turns out that class can be precisely characterized, as we now show.

We begin by summarizing the theory of hyperproperties:
\begin{definition}[Hyperproperties~\cite{Clarkson+Schneider/10/Hyperproperties}]
A \emph{trace} is a finite or infinite sequence of states.  
%(The terms ``infinite trace'' and ``path'' are therefore synonymous.)
Define $\trfin$ to be the set of finite traces and $\trinf$ to be the set of infinite traces.
A \emph{trace property} is a set of infinite traces. 
A set $T$ of traces satisfies a trace property $P$ iff $T \subseteq P$.
A \emph{hyperproperty} is a set of sets of infinite traces, or equivalently a set of trace properties. 
The interpretation of a hyperproperty as a security policy is that the hyperproperty is the set of systems allowed by that policy.
Each trace property in a hyperproperty is an allowed system, specifying exactly which executions must be possible for that system. 
Thus a set $T$ of traces satisfies hyperproperty $\hp{H}$ iff $T$ is in $\hp{H}$.
%Given a trace property $P$, the powerset of $P$ is the unique hyperproperty that expresses the same policy as $P$.  Denote that hyperproperty as $\lift{P}$.
\end{definition}

We now give a new characterization of hyperproperties in terms of their quantifier structure.
Let $Q$ be a finite sequence of universal and existential quantifiers---for example, $\forall\exists$.
Define hyperproperty \hp{H} to be an \emph{$Q$-hyperproperty} iff $|Q| = k$ and 
\begin{equation*}
\existsqer{R \subseteq \trinf^k}{\forallqer{S \in \hp{H}}
{\quant{Q}{\vec{t} \in \trinf^k}
{\mathit{set}(\vec{t}) \subseteq S}{\vec{t} \in R}{:}{:}}},
\end{equation*}
where $\trinf^k$ denotes the $k$-fold Cartesian product of $\trinf$ (i.e., the set of all $k$-tuples of infinite traces), $\vec{t}$ denotes a $k$-tuple $(t_1,\ldots,t_k)$ of traces, and $\mathit{set}(\vec{t}\;)$ denotes $\setdef{t_i}{1 \leq i \leq k}$.
Notation $Q \, \vec{t} \in \trinf^k$ is an abbreviation for $k$ nested quantifications:
\begin{equation*}
Q_1 \, t_1 \in \trinf \;\! : \;\! Q_2 \, t_2 \in \trinf \;\! : \;\! \ldots \;\! : \;\! Q_k \, t_k \in \trinf,
\end{equation*}
where $Q_i$ denotes quantifier $i$ from sequence $Q$.
For example, $\forall\exists \, \vec{t} \in \trinf^k$ abbreviates $\forall \, t_1 \in \trinf \;\! : \;\! \exists \, t_2 \in \trinf$.
For a system $S$ to be a member of $\hp{H}$, all (appropriately quantified) $k$-tuples of traces from $S$ must satisfy $R$, in which case relation $R$ \emph{defines} \hp{H}.

Noninference is a $\forall\exists$-hyperproperty.
The HyperLTL formula~\eqref{hp:noninference} that characterizes it makes this apparent.
The two quantifiers show that the policy is defined in terms of pairs of traces. 
Likewise, observational determinism~\eqref{hp:od} is a  $\forall\forall$-hyper\-property, and generalized noninterference~\eqref{hp:gni} is a $\forall\forall\exists$-hyper\-property.
All trace properties are simply $\forall$-hyperproperties.

A $Q$-hyperproperty is \emph{star-free $\omega$-regular} if its defining relation $R$ is a star-free $\omega$-regular set.
(These are like regular sets, in that they are formed with union, complementation, and concatenation; but instead of Kleene star they have the $\omega$ operator, which infinitely repeats words.)  
%Meaning that it can be expressed with the linear-time temporal connectives. 
%(Or, equivalently~\cite{GabbayPSS80}, that it can be expressed in S1S, the monadic second-order theory of one successor.)
\begin{proposition}
$\hp{H}$ is a star-free $\omega$-regular $Q$-hyperproperty iff there exists a HyperLTL formula $\phi$, such that $S \in \hp{H}$ iff $S \models \phi$.
\end{proposition}
\begin{proof}
The relation $R$ that defines $\hp{H}$ is equivalent to formula $\phi$.
That formula is definable with the linear-time connectives, therefore~\cite{GabbayPSS80} it describes a star-free $\omega$-regular set.
\end{proof}
\noindent HyperLTL therefore expresses exactly the star-free $\omega$-regular $Q$-hyper\-prop\-er\-ties, just as LTL expresses~\cite{GabbayPSS80} exactly the star-free $\omega$-regular trace properties, which are themselves $\forall$-hyperproperties.

\paragraph*{Safety.}
The characterization of HyperLTL's expressivity can be extended further.
\emph{Safety}~\cite{Alpern+Schneider/1985/DefiningLiveness} proscribes ``bad things.'' 
A bad thing is \emph{finitely observable}, meaning its occurrence can be detected in finite time, and \emph{irremediable}, so its occurrence can never be remediated by future events.
The theory of hyperproperties includes safety:

\begin{definition}[Hypersafety~\cite{Clarkson+Schneider/10/Hyperproperties}]
A hyperproperty $\hp{S}$ is a \emph{safety hyperproperty} (is
\emph{hypersafety}) iff
\begin{multline*}
\forallq{T \subseteq \trinf}{T \notin \hp{S}}{\existsq{B \subseteq \trfin }{|B| \in \mathbb{N} \andsp B \leq T \\ }{\forallq{U \subseteq \trinf}{B \leq U}{U \notin
\hp{S}}}}.
\end{multline*}
For a system $T$ that doesn't satisfy a safety hyperproperty, the bad thing is a finite set $B$ of finite traces.  
$B$ cannot be a prefix of any system $U$ satisfying the hyper safety property.
A finite trace $t$ is a \emph{prefix} of a (finite or infinite) trace $t'$, denoted $t \prefix t'$, iff $t' = tt''$ for some $t'' \in \tr$.
And a finite set $T$ of finite traces is a prefix of a (finite or infinite) set $T'$ of (finite or infinite) traces, denoted $T \leq T'$, iff $\forallqer{t \in T}{\existsqer{t' \in T'}{t \leq t'}}$.
A $k$-safety hyperproperty is a safety hyperproperty in which the bad thing never involves more than $k$ traces.
A hyperproperty $\hp{S}$ is a \emph{$k$-safety hyperproperty} (is \emph{$k$-hypersafety})~\cite{Clarkson+Schneider/10/Hyperproperties} iff
\begin{multline*}
\forallq{T \subseteq \trinf}{T \notin \hp{S}}{\existsq{B \subseteq \trfin }{|B| \leq k \andsp B \leq T\\ }{\forallq{U \subseteq \trinf}{B \leq U}{U \notin \hp{S}}}}.
\end{multline*}
\noindent This is just the definition of hypersafety but with the cardinality of $B$ bounded by $k$.
\end{definition}

Define a relation $R$ to be a \emph{$k$-safety relation} iff
\begin{multline*}%\label{eq:ksafetyrel}
\forallq{\vec{t} \in \trinf^k}{\vec{t} \not\in R}
 {\existsq{\vec{b} \in \trfin^{\leq k}}{\vec{b} \leq \vec{t}}
   {\\ \forallq{\vec{u} \in \trinf^k}{\vec{b} \leq \vec{u}}{\vec{u} \not\in R}}}.
\end{multline*}
Prefix on tuples of traces is the pointwise application of prefix on traces:  $\vec{t} \leq \vec{u}$ iff, for all $i$, it holds that $t_i \leq u_i$.
Set $\trfin^{\leq k}$ is all $n$-tuples of traces where $n \leq k$.

Observational determinism is a 2-safety hyperproperty~\cite{Clarkson+Schneider/10/Hyperproperties}, as well as a $\forall\forall$-hyperproperty definable by a 2-safety relation.  Moreover, the $k$-safety hyperproperties are all $\forall^k$-hyper\-prop\-er\-ties, where $\forall^k$ denotes a sequence of $k$ universal quantifiers:
\begin{proposition}
A $\forall^k$-hyperproperty $\hp{H}$ is definable by a $k$-safety relation iff $\hp{H}$ is a $k$-safety hyperproperty.
\end{proposition}
\begin{proof}
($\Rightarrow$) The bad thing for a system that doesn't satisfy $\hp{H}$ is tuple $\vec{b}$.
($\Leftarrow$) The relation is the set of all $k$-tuples of traces that do not contain a bad thing as a prefix.
\end{proof}
The $k$-safety hyperproperties are known~\cite{Clarkson+Schneider/10/Hyperproperties} to have a relatively complete verification methodology based on self-composition.
Our prototype model-checker in Section \ref{sec:prototype} increases the class of hyperproperties that can be verified from $k$-safety to $\forall^k$-hyperproperties and beyond to the whole class of star-free $\omega$-regular $Q$-hyperproperties.

==> intro2.tex <==
% !TEX root = paper.tex

\section{Introduction}
\label{sec:intro}

\emph{Trace properties}, which developed out of an interest in proving the correctness of
programs~\cite{Lamport77}, characterize correct behavior as 
properties of individual execution traces.
Although early verification techniques specialized in proving
individual correctness properties of interest, such as mutual
exclusion or termination, temporal logics soon emerged as a general,
unifying framework for expressing and verifying trace properties.
%Practical model-checking tools~\cite{Holzmann:1997:SPIN,NuSMV:2000:Cimatti,Esparza+Schwoon/2001/ABDDBasedModelCheckerForRecursivePrograms,Cook+Koskinen/2011/MakingPropheciesWithDecisionPredicates,Cook+Koskinen+Vardi/2011/TemporalPropertyVerificationAsAProgramAnalysisTask,Cook+Koskinen/2013/ReasoningAboutNondeterminismInPrograms} based on those logics now enable automated verification of program correctness. 
Practical model checking
tools~\cite{Holzmann:1997:SPIN,NuSMV:2000:Cimatti,Cook+Koskinen+Vardi/2011/TemporalPropertyVerificationAsAProgramAnalysisTask}
based on those logics now enable automated verification of program
correctness.

Verification of security is not directly possible with
such tools, because some important security policies cannot be characterized
as properties of individual execution traces~\cite{McLean:1994:GeneralTheory}. 
Rather, they are properties of sets of execution traces, also known as 
\emph{hyperproperties}~\cite{ClarksonS10}.
Specialized verification techniques have been developed for
particular hyperproperties~\cite{HammerS09,BanerjeeN05,Myers99},
as well as for \emph{2-safety} properties~\cite{Terauchi+Aiken/05/SecureInformationFlowAsSafetyProblem}, which 
are properties of pairs of execution traces. 
But a unifying program logic for expressing and verifying
hyperproperties could enable automated verification of a
wide range of security policies.

In this paper, we propose two such logics.
Both are based, like
hyperproperties, on examining more than one execution trace at a time.
Our first logic, \emph{HyperLTL}, generalizes linear-time temporal
logic (LTL)~\cite{Pnueli:1977:TLP}.  LTL implicitly quantifies over
only a single execution trace of a system, but HyperLTL allows
explicit quantification over multiple execution traces simultaneously,
as well as propositions that stipulate relationships among those
traces.  For example, HyperLTL can express information-flow
policies such as \emph{observational 
determinism}~\cite{McLean92,Roscoe95,ZdancewicM03}, which requires
programs to behave as (deterministic) functions from low-security
inputs to low-security outputs.  The following two programs do not
satisfy observational determinism, because they leak the value of
high-security variable $h$ through low-security variable $l$, thus making
the program behave nondeterministically from a low-security users's
perspective:
%
\begin{equation*}
\begin{array}{l@{\hspace{4em}}l}
\text{(1)}~~l := h & \text{(2)}~~\cond{h=0}{l:=1}{l:=0}
\end{array}
\end{equation*}
%
Other program logics could already express observational determinism or closely related policies~\cite{BartheDR04,HuismanWS/06/TLCharacterisationOfOD}.
But HyperLTL provides a unifying logic in which many information-flow security policies
can be directly expressed.   

Information-flow policies are not one-size-fits-all.  Different policies might be needed 
depending on the power of the adversary. For example, the following
program does not satisfy observational determinism, but the program might be
acceptable if nondeterministic choices, denoted $\talloblong$, are
resolved such that the probability distribution on output value $l$ is
uniform:
%
\begin{equation*}
\text{(3)} ~~ l := h ~\talloblong~ l := 0 ~\talloblong~ l := 1
\end{equation*}
%
On the other hand, if the adversary can influence the resolution of nondeterministic choices, program (3) could be exploited to leak information.
Similarly, the following program does satisfy observational
determinism, but the program might be unacceptable if adversaries 
can monitor execution time:
%
\begin{equation*}
\text{(4)} ~~ \while{h > 0}{\{h := h-1\}}
\end{equation*}%
%
\setcounter{equation}{4}%% LaTeX: for later unique labeling of equations
%
In Section~\ref{sec:examples}, we show how policies appropriate for the above 
programs, as well as other security policies, can be formalized in HyperLTL.  


%We also study the class of hyperproperties
%expressible in HyperLTL, and show that this class contains the
%linear-time
%2-safety~\cite{Terauchi+Aiken/05/SecureInformationFlowAsSafetyProblem}
%and $k$-safety~\cite{Clarkson+Schneider/10/Hyperproperties}
%hyperproperties as special cases.

Our second logic, \emph{\Hpctl{}}, generalizes a branching-time
temporal logic,
\ctlstr{}~\cite{EmersonH86}.
Although \ctlstr{} already has explicit trace quantifiers,
only one trace is ever in scope at a given point in a formula (see
Section~\ref{sec:ltlctl}),
so \ctlstr{} cannot directly express hyperproperties.
%(Even the modal $\mu$-calculus cannot express all hyperproperties~\cite{Alur+Cerny+Zdancewic/06/PreservingSecrecy}.)
But \Hpctl{} can, because it permits quantification over multiple 
execution traces simultaneously.
HyperLTL and \Hpctl{} enjoy a similar relationship to that of LTL and \ctlstr{}:
HyperLTL is the syntactic fragment of \Hpctl{} containing only formulas in \emph{prenex} form---that is, formulas that begin exclusively with quantifiers and end with a quantifier-free formula.
\Hpctl{} is thus a strict generalization of HyperLTL.
\Hpctl{} also generalizes a related temporal logic, SecLTL~\cite{Dimitrova:2012:SecLTL}, and subsumes epistemic temporal logic~\cite{Fagin-book-95,Meyden/1993/AxiomsForKnowledgeAndTimeInDistributedSystemsWithPerfectRecall} (see Section~\ref{sec:relatedlogics})\footnote{%
Milushev and Clarke~\cite{MilushevC12,Milushev:2013:thesis,MilushevC13} have also
proposed logics for hyperproperties, based on the polyadic $\mu$-calculus, which we discuss in Section~\ref{sec:relatedwork}.}. 
%Although we do not yet know which of \Hpctl{} or epistemic temporal logic is strictly more expressive, we do know that the model-checking problem for \Hpctl{} enjoys lower worst-case complexity.
%\Hpctl{} makes it easy to directly formulate information-flow policies from the literature, rather than having to encode those policies with connectives for information hiding (as in SecLTL) or for knowledge (as in epistemic temporal logic).

Having defined logics for hyperproperties, we investigate model-checking of those logics. 
In Section~\ref{sec:ctlmodelchecking}, we show that for \Hpctl{} the 
model-checking problem is decidable by reducing it to the 
satisfiability problem for quantified propositional temporal 
logic (QPTL)~\cite{Sistla+Vardi+Wolper/1987/TheComplementationProblemForBuchiAutomata}. 
Since \Hpctl{} generalizes HyperLTL, we immediately obtain that the HyperLTL model-checking
problem is also decidable. 
We present a hierarchy of fragments, which allows us to precisely characterize the complexity of the model-checking problem in the number quantifier alternations. 
The lowest fragment, which disallows any quantifier alterantion, can be checked by a space-efficient polynomial-time algorithm (NLOGSPACE in the number of states of the program). 

We also prototype a model
checker that can handle an important fragment of HyperLTL, including all the
examples from Section~\ref{sec:examples}.  The prototype implements a
new model-checking algorithm 
based on a well-known LTL algorithm~\cite{Vardi:1994:infComp,Wolper00} and on
a self-composition construction~\cite{BartheDR04,Terauchi+Aiken/05/SecureInformationFlowAsSafetyProblem}. 
The complexity of our algorithm is exponential in the size of
the program and doubly exponential in the size of the
formula---impractical for real-world programs, but at least a
demonstration that model-checking of hyperproperties formulated in our logic is possible.

This paper contributes to theoretical and foundational aspects of security by:
\begin{compactitem}
\item defining two new program logics for expressing hyperproperties,
\item demonstrating that those logics are expressive enough to formulate important in\-for\-ma\-tion-flow policies, 
\item proving that the model checking problem is decidable, and
\item prototyping a new model checking algorithm and using it to verify security policies.
\end{compactitem}

The rest of the paper is structured as follows.  Section
\ref{sec:hyperltl} defines the syntax and semantics of HyperLTL.
Section~\ref{sec:examples} provides several example formulations of
information-flow policies.
%\S\ref{sec:hp} discusses hyperproperties and HyperLTL.
Section~\ref{sec:hyperctl} defines the syntax and semantics of
\Hpctl{}.  Section~\ref{sec:relatedlogics} compares our two logics
with other temporal and epistemic logics.
Section~\ref{sec:ctlmodelchecking} obtains a model checking algorithm
for \Hpctl{}.  Section~\ref{sec:prototype} describes our prototype
model checker.  Section~\ref{sec:relatedwork} reviews related work,
and Section~\ref{sec:conclusion} concludes.



==> mcleans.tex <==
% !TEX root = paper.tex
\section{Formalization of security policies in SIF}
\label{app:mcleans}

\emph{Selective Interleaving Functions framework}~\cite{McLean:1994:GeneralTheory} is introduced by John McLean for formal presentation and analysis of information-flow policies. This framework in mainly developed for state-based systems. Policies expressed in SIFs can be easily converted to HyperLTL and verified. We show the formalization of several policies of Section~\ref{sec:examples} in selective interleaving functions framework.

Consider two security levels of high and low. Every state in the system is of the form $\<\<in_1,\dots,in_m\>,\<out_1,\dots,out_n\>\>$, where $in$ and $out$ denote input and output respectively. We order inputs and outputs in a way that inputs/outputs of high users are at first, and then comes the inputs/outputs of low users. Therefore, we can show a state by $\<\<highin:lowin\>,\<highout:lowout\>\>$. The values of inputs and outputs are from the set $\{0,1,\lambda\}$, where $\lambda$ means no input or no output. Let $\Sigma$ be the two-level security state space. We define $trace(\Sigma)$ to be the set of all sequence of states over $\Sigma$ (note that trace here is defines as the sequence of states, different from the definition of traces in Section~\ref{sec:hyperltl}.)

\paragraph{Noninference.} 
Let $purge: trace(\Sigma)\rightarrow trace(\Sigma)$ be the purge function, which sets all high input and output variables of a trace to $\lambda$:
\begin{eqnarray*}
	purge(t)&=& \<\<\lambda^H:lowin(t)[0]\>,\<\lambda^H:lowout(t)[0]\>\> \\
			&& \<\<\lambda^H:lowin(t)[1]\>,\<\lambda^H:lowout(t)[1]\>\>\dots
\end{eqnarray*}

where $\lambda^H=\lambda,\dots,\lambda$ is of the same length as high inputs when is set as high inputs, or high outputs when set as high outputs. $lowin(t)$ and $lowout(t)$ are the sequence of low inputs and low outputs of trace $t$ respectively.

A set of traces $T$ satisfies noninference if the set is closed under $purge$. That is, for all traces $t\in T$, we have $purge(t)\in T$.

\paragraph{Generalized noninterference.}

A function $f:trace(\Sigma)\times trace(\Sigma)\rightarrow trace(\Sigma)$ is an \emph{input interleaving} iff $f(t_1,t_2) = t$ then
\begin{eqnarray*}
	highin(t)=highin(t_1), lowin(t)=lowin(t_2), \text{ and } lowout(t)=lowout(t_2)
\end{eqnarray*}

A set of traces $T$ satisfies generalized noninference if the set is closed under input interleaving. That is, for all traces $t_1,t_2\in T$, we have $f(t_1,t_2)\in T$.

Other properties---for example, generalized noninference, deducibility security, and separability---that have a formalization in SIF framework can likewise formulated in HyperLTL.

==> semantics.tex <==
% !TEX root = paper.tex

\section{Semantics}
\label{sec:semantics}

HyperLTL formulas are interpreted with respect to \emph{computations}.
A computation abscessts away from the states in a path, representing each state by the propositions that hold of that state.
Let $\Atoms$ denote the set of atomic propositions. 
Formally, a computation $\gamma$ is an infinite sequence over $\powerset(\Atoms)$, where $\powerset$ denotes the powerset operator.
Define $\gamma[i]$ to be element $i$ of computation $\gamma$.  
Hence, $\gamma[i]$ is a set of propositions.
And define $\gamma[i..]$ to be the suffix of $\gamma$ starting with element $i$---that is, the sequence $\gamma(i)\gamma(i+1)\ldots$
We index sequences starting at 1, so $\gamma[1..] = \gamma$.

A computation represents a single path, but HyperLTL formulas may quantify over multiple paths.
To represent that, let $\Gamma$ denote a finite tuple $(\gamma_1,\dots,\gamma_k)$ of computations.
Define $|\Gamma|$ to be the length $k$ of $\Gamma$,
and define projection $\proj_i(\Gamma)$ to be element $\gamma_i$.
Given a tuple $\Gamma$ define $\Gamma\cdot\gamma$ to be the concatenation of element $\gamma$ to the end of tuple $\Gamma$, yielding tuple $(\gamma_1,\dots,\gamma_k,\gamma)$.
Extend that notation to concatenation of tuples by defining  $\Gamma\cdot\Gamma'$ to be the tuple containing all the elements of $\Gamma$ followed by all the elements of $\Gamma'$.
Extend notations $\gamma[i]$ and $\gamma[i..]$ to apply to computation tuples by defining $\Gamma[i] = (\gamma_1[i],\dots,\gamma_k[i])$---that is, the tuple containing element $i$ from each computation in $\Gamma$---and $\Gamma[i..] = (\gamma_1[i..],\dots,\gamma_k[i..])$.

HyperLTL formulas may involve propositions over multiple states.  
For example, $\atom{low-equiv}$ in the definition of noninference~\eqref{hp:ni} holds when two states have the same low inputs and outputs. 
We therefore need a means to determine what \emph{compound} propositions hold of a tuple of states, given what atomic propositions hold of the individual states.
To do that, we introduce \emph{bonding} functions that describe how to produce compound propositions out of tuples of atomic propositions.
Let $\Compounds$ denote the set of compound propositions, and assume that $\Atoms \subseteq \Compounds$. 
Let $B$ be a family $\setdef{B_i}{i\in\mathbb{N}}$ of functions, such that each $B_i$ is a function from $\mathcal{P}(\Atoms)^i$ to $\mathcal{P}(\Compounds)$.
Notation $X^n$ is the $n$-ary cartesian power of set $X$.
We require $B_1$ to be the identity function, so that length-1 tuples are not changed by bonding.
As an example, consider a bonding function $B_2$ that describes when two states are low-equivalent.
Given a set $\setdef{\atom{low}_i}{1 \leq i \leq n}$ of atoms, describing $n$ different low states, we could define $B_2$ such that $B_2(\{\atom{low}_i\},\{\atom{low}_i\}) = \{\atom{low-equiv}\}$, and $B_2(\{\atom{low}_i\},\{\atom{low}_j\}) = \emptyset$ if $i \neq j$.
Given a tuple, it is always clear from the length of the tuple which function $B_i$ should be applied to it, so henceforth we omit the subscript.

The validity judgment for HyperLTL formulas is written $\Gamma \models \phi$.  
Formula $\phi$ must be well-formed.
The judgment implicitly uses a \emph{model} $M$, which is a set of computations, and a family $B$ of bonding functions.
We omit notating $M$ and $B$ as part of the judgment, because they do not vary during the interpretation of a formula.  
Validity is defined as follows:
\begin{enumerate}
\item\label{validity:A} $\Gamma \models \A\psi$ iff for all $\gamma\in M : \Gamma\cdot\gamma\models\psi$ 
\item\label{validity:E} $\Gamma \models \E\psi$ iff there exists $\gamma\in M : \Gamma\cdot\gamma\models\psi$
\item\label{validity:p} $\Gamma \models p$ iff $p \in B(\Gamma[1])$
\item\label{validity:not} $\Gamma \models \neg \psi$ iff $\Gamma\not\models \psi$ 
\item\label{validity:or} $\Gamma \models \psi_1\vee\psi_2$ iff $\Gamma \models\psi_1$ or $\Gamma\models \psi_2$
\item\label{validity:focus} $\Gamma \models \<\psi_1,\dots,\psi_n\>$ iff for all $i$ : if $1 \leq i \leq n$ then $\proj_i(\Gamma)\models\psi_i$ 
\item\label{validity:X} $\Gamma \models \X\psi$ iff $\Gamma[2..]\models\psi$
\item\label{validity:U} $\Gamma \models \psi_1\U\psi_2$ iff there exists $k : k \geq 1$ and $\Gamma[k..]\models\psi_2$ and for all $j$ : if $1 \leq j < k$ then $\Gamma[j..] \models\psi_1$
\end{enumerate}
Clauses \ref{validity:A} and \ref{validity:E} quantify over a computation $\gamma$ from $M$, and they concatenate $\gamma$ to $\Gamma$ to evaluate subformula $\psi$.
Clause \ref{validity:p} means satisfaction of atomic propositions is determined by the first element of each computation in $\Gamma$.
Clauses \ref{validity:not} and \ref{validity:or} are standard.
In clause \ref{validity:focus}, elements of a focus formula are independently evaluated over their corresponding individual computations.
Clauses \ref{validity:X} and \ref{validity:U} are the standard LTL definitions of $\X$ and $\U$, upgraded to work over a sequence of computations.


